Sounding-Based Evaluation of Multi-Sensor ISAC Networks for Drone Applications: Measurement and Simulation Perspectives

With the upcoming multitude of commercial and public applications envisioned in the mobile 6G radio landscape using unmanned aerial vehicles (UAVs), integrated sensing and communication (ISAC) plays a key role to enable the detection and localization of passive objects with radar sensing, while optimizing the utilization of scarce resources. To explore the potential of future ISAC architectures with UAVs as mobile nodes in distributed multi-sensor networks, the system's fundamental capability to detect static and dynamic objects that reveal themselves by their bi-static back-scattering needs to be evaluated. Therefore, this paper addresses simulation- and measurement based data acquisition methods to gather knowledge about the bistatic reflectivity of single objects including their Micro-Doppler signature for object identification as well as the influence of multipath propagation in different environments on the localization accuracy and radar tracking performance. We show exemplary results from simulation models, bi-static reflectivity measurements in laboratory environment and real-flight channel sounding experiments in selected scenarios showcasing the potential of synthetic and measured data sets for development and evaluation of ISAC algorithms. The presented measurement data sets are publicly available to encourage the academic RF community to validate future algorithms using realistic scenarios alongside simulations models.

==> Makefile <==
BUILD_DIR=build
SHELL=/bin/sh
NAME=paper

default: full

.PHONY: clean
clean:
	rm -f arxiv.zip
	@ if [ -h $(BUILD_DIR) ] ; then \
		rm -rf `readlink $(BUILD_DIR)` ;\
		rm $(BUILD_DIR) ;\
	else \
		rm -rf $(BUILD_DIR) ;\
	fi

$(BUILD_DIR):
	@ if [ -h $(BUILD_DIR) ] ; then rm $(BUILD_DIR) ; fi
	ln -s `mktemp -d /tmp/$(NAME)-build.XXXXXXXX` $(BUILD_DIR)
	chmod 700 `readlink $(BUILD_DIR)`

.PHONY: full
full: $(NAME).tex $(BUILD_DIR)
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<
	BIBINPUTS="$(BUILD_DIR):" TEXMFOUTPUT="$(BUILD_DIR):" bibtex $(BUILD_DIR)/$(NAME)
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<

.PHONY: quick
quick: $(NAME).tex $(BUILD_DIR)/$(NAME).aux
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<

arxiv.zip: $(NAME).tex $(BUILD_DIR)/ Figures/
	cp -a $(BUILD_DIR)/$(NAME).bbl .
	zip -r arxiv.zip $(NAME).tex $(NAME).bbl orcidlink.sty Figures/
	rm $(NAME).bbl

